Towards Practical Physics-Informed ML Design and Evaluation for Power Grid

When applied to a real-world safety critical system like the power grid, general machine learning methods suffer from expensive training, non-physical solutions, and limited interpretability. To address these challenges for power grids, many recent works have explored the inclusion of grid physics (i.e., domain expertise) into their method design, primarily through including system constraints and technical limits, reducing search space and defining meaningful features in latent space. Yet, there is no general methodology to evaluate the practicality of these approaches in power grid tasks, and limitations exist regarding scalability, generalization, interpretability, etc. This work formalizes a new concept of physical interpretability which assesses how a ML model makes predictions in a physically meaningful way and introduces an evaluation methodology that identifies a set of attributes that a practical method should satisfy. Inspired by the evaluation attributes, the paper further develops a novel contingency analysis warm starter for MadIoT cyberattack, based on a conditional Gaussian random field. This method serves as an instance of an ML model that can incorporate diverse domain knowledge and improve on these identified attributes. Experiments validate that the warm starter significantly boosts the efficiency of contingency analysis for MadIoT attack even with shallow NN architectures.

==> Biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures_bio/bio_Shimiao.jpg}}] 
{Shimiao Li} received the B.E. degree in electrical engineering
from Tianjin University, China, in 2018. She is currently a Ph.D. candidate in the Department of Electrical and Computer Engineering (ECE) at Carnegie
Mellon University, where she is advised by Lawrence Pileggi. Her research interests include analytical methods for grid operation and optimization, as well as physics-informed machine learning for real-world grid cyber-security, reliability and optimization appliations.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures_bio/bio_Amrit.jpg}}] 
{Amritanshu Pandey} was born in Jabalpur, India. He received the M.Sc. and Ph.D. degree in Electrical Engineering in 2012 and 2019, respectively, from Carnegie Mellon University, Pittsburgh, PA, USA. He is currently a Special Faculty in the Electrical and Computer Engineering department at Carnegie Mellon University. He has previously worked at Pearl Street Technologies, Inc. as Senior Research Scientist and as an Engineer at MPR Associates, Inc. He develops first principles-based physics driven and ML-based data driven methods and models for energy systems that are expressive (i.e., capture sufficient physical behavior accurately) and efficient in terms of speed and scalability.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures_bio/bio_larry.jpg}}] 
{Lawrence Pileggi} is the Tanoto professor and Head of electrical and computer engineering at Carnegie Mellon University, and has previously held positions at Westinghouse Research and Development and the University of Texas at Austin. He received his Ph.D. in Electrical and Computer Engineering from Carnegie Mellon University in 1989. His research interests include various aspects of digital and analog integrated circuit design, and simulation, optimization and modeling of electric power systems. He was a co-founder of  Fabbrix Inc., Extreme DA, and Pearl Street Technologies. He has received various awards, including Westinghouse corporation’s highest engineering achievement award, the Semiconductor Research Corporation (SRC) Technical Excellence Awards in 1991 and 1999, the FCRP inaugural Richard A. Newton GSRC Industrial Impact Award, the SRC Aristotle award in 2008, the 2010 IEEE Circuits and Systems Society Mac Van Valkenburg Award, the ACM/IEEE A. Richard Newton Technical Impact Award in Electronic Design Automation in 2011, the Carnegie Institute of Technology B.R. Teare Teaching Award for 2013, and the 2015 Semiconductor Industry Association (SIA) University Researcher Award. He is a co-author of "Electronic Circuit and System Simulation Methods," McGraw-Hill, 1995 and "IC Interconnect Analysis," Kluwer, 2002. He has published over 400 conference and journal papers and holds 40 U.S. patents. He is a fellow of IEEE.
\end{IEEEbiography}
